Hardware Implementation of Task-based Quantization in Multi-user Signal Recovery

Quantization plays a critical role in digital signal processing systems, allowing the representation of continuous amplitude signals with a finite number of bits. However, accurately representing signals requires a large number of quantization bits, which causes severe cost, power consumption, and memory burden. A promising way to address this issue is task-based quantization. By exploiting the task information for the overall system design, task-based quantization can achieve satisfying performance with low quantization costs. In this work, we apply task-based quantization to multi-user signal recovery and present a hardware prototype implementation. The prototype consists of a tailored configurable combining board, and a software-based processing and demonstration system. Through experiments, we verify that with proper design, the task-based quantization achieves a reduction of 25 fold in memory by reducing from 16 receivers with 16 bits each to 2 receivers with 5 bits each, without compromising signal recovery performance.

==> Hardware Implementation of Task-based Quantization in Multi-user Signal Recovery/definitions.tex <==

\newcommand{\df}{d_\mathrm{F}}

\newcommand{\xf}{x_\mathrm{F}}
\newcommand{\yf}{y_\mathrm{F}}
\newcommand{\zf}{z_\mathrm{F}}


\newcommand{\g}{\mathrm{g}}
\newcommand{\Ge}{G_\mathrm{e}}

\newcommand{\p}{\mathbf{p}}
\newcommand{\hpf}{\hat{\mathbf{p}}_\mathrm{F}}
\newcommand{\pf}{\mathbf{p}_\mathrm{F}}
\newcommand{\pil}{\mathbf{p}_{i,l}}
\newcommand{\yil}{{y}_{i,l}}
\newcommand{\Yil}{{Y}_{i,l}}
\newcommand{\Ail}{{A}_{i,l}}
